Automating Rigid Origami Design

Rigid origami has shown potential in large diversity of practical applications. However, current rigid origami crease pattern design mostly relies on known tessellations. This strongly limits the diversity and novelty of patterns that can be created. In this work, we build upon the recently developed principle of three units method to formulate rigid origami design as a discrete optimization problem, the rigid origami game. Our implementation allows for a simple definition of diverse objectives and thereby expands the potential of rigid origami further to optimized, application-specific crease patterns. We showcase the flexibility of our formulation through use of a diverse set of search methods in several illustrative case studies. We are not only able to construct various patterns that approximate given target shapes, but to also specify abstract, function-based rewards which result in novel, foldable and functional designs for everyday objects.

==> figures/results_a_figure.tex <==
\setlength{\wimg}{0.2\textwidth}
\begin{landscape}
\begin{figure*}[t]

    % legend
    \hspace*{0.2cm}
    \rowlegend{ }
    \hspace{-0.6cm}
    \begin{minipage}{1.5\textwidth}
    TARGET
    \hspace{1.4cm}
    \vspace{0.1cm}
    RDM 
    \hspace{1.2cm}
    \vspace{0.1cm}
    PPO MLP
    \hspace{0.6cm}
    \vspace{0.1cm}
    PPO ResNet
    \hspace{1cm}
    \vspace{0.1cm}
    DFTS
    \hspace{1.6cm}
    \vspace{0.1cm}
    BFTS
    \hspace{1.5cm}
    \vspace{0.1cm}
    MCTS
    \end{minipage}
    
    
    % cube
    \hspace*{0.2cm}
    \rowlegend{cube}
    \hspace{-1cm}
    \begin{minipage}{1.5\textwidth}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/cube_target.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/cube_RDM.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/cube_PPO_MLP.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/cube_PPO_ResNet.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/cube_DFTS.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/cube_BFTS.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/cube_MCTS.png}
    \end{minipage}


    % pyramid
    \hspace*{0.2cm}
    \rowlegend{pyramid}
    \hspace{-1cm}
    \begin{minipage}{1.5\textwidth}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/pyramid_target.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/pyramid_RDM.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/pyramid_PPO_MLP.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/pyramid_PPO_ResNet.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/pyramid_DFTS.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/pyramid_BFTS.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/pyramid_MCTS.png}
    \end{minipage}
    
    
    % bowl
    \hspace*{0.2cm}
    \rowlegend{bowl}
    \hspace{-1cm}
    \begin{minipage}{1.5\textwidth}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/bowl_target.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/bowl_RDM.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/bowl_PPO_MLP.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/bowl_PPO_ResNet.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/bowl_DFTS.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/bowl_BFTS.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/bowl_MCTS.png}
    \end{minipage}
  
  
    % face
    \hspace*{0.2cm}
    \rowlegend{face}
    \hspace{-1cm}
    \begin{minipage}{1.5\textwidth}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/face_target.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/face_RDM.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/face_PPO_MLP2.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/face_PPO_ResNet2.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/face_DFTS.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/face_BFTS.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_a/face_MCTS.png}
    \end{minipage}
  
    \caption{The figure shows the best shapes across the experiments on four target shapes.}
    \vspace{-0.3cm}
    \label{fig:results_a}

\end{figure*}
\end{landscape}

==> figures/results_b_figure.tex <==
\setlength{\wimg}{0.3\textwidth}

\begin{figure*}[t]

    
    
    % 5/6pi 
    \hspace*{0.2cm}
    \rowlegend{$5/6\pi$}
    \hspace{-1cm}
    \begin{minipage}{1.5\textwidth}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_b/table_00.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_b/table_01.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_b/table_02.png}
    \vspace{0.1cm}
    \end{minipage}


    % 4/5pi 
    \hspace*{0.2cm}
    \rowlegend{$4/5\pi$}
    \hspace{-1cm}
    \begin{minipage}{1.5\textwidth}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_b/table_10.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_b/table_11.png}
    \vspace{0.1cm}
    \end{minipage}
    
    
    % 2/3pi 
    \hspace*{0.2cm}
    \rowlegend{$2/3\pi$}
    \hspace{-1cm}
    \begin{minipage}{1.5\textwidth}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_b/table_20.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_b/table_21.png}
    \vspace{0.1cm}
    \includegraphics[width=\wimg]{figures/results_b/table_22.png}
    \vspace{0.1cm}
    \end{minipage}
  
  
    \caption{The eight highest return imaginations of a table from left to right, the activation angle $\psi$ being row-wise fixed.}
    \vspace{-0.3cm}
    \label{fig:results_b_figure}

\end{figure*}
